Flotta: a Secure and Flexible Spark-inspired Federated Learning Framework

We present Flotta, a Federated Learning framework designed to train machine learning models on sensitive data distributed across a multi-party consortium conducting research in contexts requiring high levels of security, such as the biomedical field. Flotta is a Python package, inspired in several aspects by Apache Spark, which provides both flexibility and security and allows conducting research using solely machines internal to the consortium. In this paper, we describe the main components of the framework together with a practical use case to illustrate the framework's capabilities and highlight its security, flexibility and user-friendliness.

==> old/old_pieces_of_text.tex <==
%\section{Background}
%\label{sec:background}

%In this section, we provide a few examples of well-known FL frameworks and we introduce our new framework, \FLib, outlining a specific need encountered in our research activities and how \FLib addresses it. 

%\subsection{FL frameworks}

%TensorFlow Federated \cite{tff2021}, developed by Google, is probably the most used FL framework at the moment, and it has an emphasis on deep learning. The IBM FL library \cite{ludwig2020ibm} supports a variety of machine learning algorithms and provides tools for model aggregation, performance evaluation, and deployment. Substra \cite{galtier2019substra}, unlike the previous two frameworks, implements decentralized training facilitated by smart contracts.

%Within open-source frameworks, Flower \cite{beutel2020flower} emphasizes simplicity and scalability. It provides an intuitive programming interface and efficient communication protocols, streamlining the process of building and deploying FL systems across multiple nodes. PySyft \cite{ziller2021pysyft}, developed by OpenMined, is another open-source framework specifically focused on deep learning, extending PyTorch. It places a strong emphasis on privacy and security, offering the possibility to use various \textit{homomorphic encryption} and \textit{secure multiparty computation} protocols.

%Beyond frameworks, ready-to-use solutions accessible via user-friendly web interfaces also exist, allowing for practical creation and management of consortia. An example of this is FeatureCloud \cite{matschinske2023featurecloud} and sfkit \cite{mendelsohn2023sfkit}, both developed for the biomedicine domain. FeatureCloud offers a variety of ready-to-use algorithms ranging from linear regression to genomic-specific ones, along with the flexibility for users to develop custom algorithms. On the other hand, sfkit specializes in genomic analysis, providing a small selection of algorithms while enforcing privacy protection through encryption techniques relying on the Lattigo library \cite{lattigo}.
